Long-tailed Classification from a Bayesian-decision-theory Perspective

Long-tailed classification poses a challenge due to its heavy imbalance in class probabilities and tail-sensitivity risks with asymmetric misprediction costs. Recent attempts have used re-balancing loss and ensemble methods, but they are largely heuristic and depend heavily on empirical results, lacking theoretical explanation. Furthermore, existing methods overlook the decision loss, which characterizes different costs associated with tailed classes. This paper presents a general and principled framework from a Bayesian-decision-theory perspective, which unifies existing techniques including re-balancing and ensemble methods, and provides theoretical justifications for their effectiveness. From this perspective, we derive a novel objective based on the integrated risk and a Bayesian deep-ensemble approach to improve the accuracy of all classes, especially the "tail". Besides, our framework allows for task-adaptive decision loss which provides provably optimal decisions in varying task scenarios, along with the capability to quantify uncertainty. Finally, We conduct comprehensive experiments, including standard classification, tail-sensitive classification with a new False Head Rate metric, calibration, and ablation studies. Our framework significantly improves the current SOTA even on large-scale real-world datasets like ImageNet.

==> rebuttal.tex <==
\subsection{Summary Response}
We thank all reviewers for their constructive comments. We understand that this paper contains many theoretical and technical details that may be hard to present in a straightforward manner, leading to some confusion and misunderstandings among reviewers. We will do our best to improve the clarity according to reviewers' comments, and will further include the experimental results on iNaturalist and more baselines. However, we would like to emphasize that despite the need for improvement in presentation, the paper's significance and novelty should not be overlooked:

- This paper is the first to formulate long-tailed classification under Bayesian Decision Theory, providing a fresh perspective and unifying key components of long-tailed problems within a single principled framework. It is non-trivial to do so and is in itself a really valuable and novel contribution. 

- Under this new framework, we propose a novel objective with utility functions, repulsive regularization, and an efficient particle optimization method, significantly enhancing the model's flexibility (user-designed utility) and reliability (predictive uncertainty).

- For real-world applications, we design the tail-sensitive utility for the risky misclassification in tailed classes, and design a new metric to evaluate this kind of risk accordingly. 

- We have compared our method with several recent baselines on large-scale datasets such as ImageNet-LT, in terms of generalization accuracy, uncertainty estimation and False Head Rate (FHR), clearly demonstrating the empirical effectiveness of our framework on various tasks.

We hope reviewers will consider our response and the significance of this work in their final assessment.

\subsection{ZyA5[54]}
Thanks for your constructive comments!

Q1: The technological innovation of the proposed method is limited.

A1: We would like to reiterate the technical contributions of our paper, which we believe demonstrate sufficient novelty:

- A new loss objective: integrated risk, which unifies data distribution, posterior inference, and decisions--three key factors in long-tailed classification. (Line 110-130)
- A novel repulsive regularization based on the entropy of variational distribution. This is different from existing diversity regularization in the multi-experts frameworks [3,4], and is more principled and naturally derived from the Bayesian framework. (Section 5.3)
- A new particle-based variational inference method without using kernels, making it easy and cheap to implement for large-scale deep models and further enabling uncertainty quantification. (Section 5.2)
- The first to consider decision loss in long-tailed problems, including new utility matrices and a new False Head Rate (FHR) metric, accounting for the cost of various types of misclassification. (Section 6.3)

Therefore, this paper makes several technical contributions to different parts in the long-tailed framework, ranging from the loss function to posterior inference and decision-making.

Q2: The first Equation in Section 5.1 is confusing.

A2: Thanks for pointing out the confusion! We will change the formula to
$$\frac{p_{test}(x,y)}{p_{train}(x,y)}=\frac{p_{test}(y)p_{test}(x|y)}{p_{train}(y)p_{train}(x|y)}=\frac{p_{test}(y)}{p_{train}(y)}$$
for clarification. Such a change does not affect the algorithm, analysis or experimental results in the paper, and is consistent with the assumption in [5].

Q3: The evaluation is not comprehensive.

A3: We follow the baseline choices in recent papers [3,4] (ICLR 2021 and CVPR 2022). We have used three datasets including ImageNet-LT, and the dataset choices also follow recent works [4,6] (CVPR 2022 and NeurIPS 2019), which do not use iNaturalist. We add an experiment on iNaturalist and the model architecture follows RIDE [3]. The accuracy is 72.3\%, which is comparable to RIDE (72.2\%). This is just a preliminary result we can get given the short rebuttal time. We will add full results in the final version. 

In summary, we have compared our method with five baselines on three datasets, including large-scale ImageNet-LT. Our method has outperformed all methods on all datasets and we believe our evaluation is comprehensive enough to demonstrate our advantages. However, we acknowledge that we did not compare with [1,2] and did not use iNaturalist. We will update related works and add full results on iNaturalist in the revision.

Q4: The related Bayesian work [7] should be added.

A4: The mentioned [7] is significantly different from our method. [7] adds Gaussian noise to Stochastic Weight Averaging (SWA) to obtain stochastic representation, while we frame the long-tailed problem from the Bayesian decision theory. Neither Gaussian noise nor SWA is used in our paper.
Besides, [7] was published after the submission deadline of ICML, so we cannot discuss it in the submitted version. We will include [7] in the final version. 

[1] Class balanced loss based on effective number of samples, CVPR 2019.

[2] On model calibration for long-tailed object detection and instance segmentation, NeurIPS 2021.

[3] Long-tailed recognition by routing diverse distribution-aware experts, ICLR 2021.

[4] Trustworthy Long-Tailed Classification, CVPR 2022.

[5] Disentangling Label Distribution for Long-tailed Visual Recognition, CVPR 2021.

[6] Learning Imbalanced Datasets with Label-Distribution-Aware Margin Loss, NeurIPS 2019.

[7] Decoupled Training for Long-Tailed Classification With Stochastic Representations, ICLR 2023.

\subsection{q19M[44]}
Thanks for the thoughtful comments!

Q1: The motivation of using Bayesian Decision Theory is unclear.

A1: The motivation is that Bayesian Decision Theory is particularly suitable for long-tailed problems. With Bayesian Decision Theory, the three key factors in long-tailed problems--data distribution, posterior inference and decision-making--can be unified into a single framework in a principled way (Line 112-128). In our paper, we have shown how this framework unifies existing techniques and provides theoretical justifications for their effectiveness (Line 267-274). This approach has enabled us to propose a new loss objective and repulsive regularization techniques, which have improved significantly over previous methods on test accuracy, False Head Rate and uncertainty estimation (Section 6).

Q2: The baseline methods considered in the experimental section are outdated and the authors should compare it to more recent baseline methods, such as ACE [1], RIDE [2], and SADE [3].

A2: We follow the baseline choices in recent papers [2,4] (ICLR 2021 and CVPR 2022). For your listed baselines, there are a few things to clarify:

- RIDE [2] is already compared as a baseline in Table 1\&2\&3 (Section 6). We did not miss it.
- Our method still outperforms [1,2,3], especially on the accuracy of tailed classes. For example, using 3 experts on CIFAR-100-LT, the tail accuracies are: ACE [1] 23.5, RIDE [2] 23.9, SADE [3] 29.3, and LBD (ours) 30.34

We will add the mentioned baselines in the final version. However, we would like to highlight that we compared our method with five baselines, including a very recent method from CVPR 2022, on three datasets, including the large-scale ImageNet-LT. Our method outperforms all the other methods on all the datasets, which we believe provides strong evidence of its effectiveness.

Q3: How to define the utility functions of different tasks?

A3: The utility function measures the gain of making different decisions (i.e., the predicted labels in long-tailed classification) and can encode our preference for high classification accuracy. For example, the two utility functions in Section 4.1 both encode their preference by assigning the highest utility to correct classification (but different gains for misclassification). Empirically, we demonstrated in Table 5 that our utility function can achieve high accuracy and account for different misclassification losses.

The utility function is a standard component in Decision Theory and its design has been studied in the literature. For example, Chapter 2.2 of [5] shows that the utility function is guaranteed to exist assuming the rationality of the decision-makers. 

To summarize, the utility function is flexible, theoretically-justified, and can be designed according to different long-tailed problems and applications. This allows us to deal with not only standard accuracy but also many different metrics (e.g., False Head Rate) that we really care about in real-world applications.

Q4: The authors should analyze the differences between their proposed method and [3].

A4: We would like to clarify that "inference" in our context refers to Bayesian inference (i.e., inferring the posterior of model parameters), which is different from the inference considered in [3] (i.e., the inference of labels on test data). 

The goals of our paper and [3] are quite different. While [3] considers the problem of unknown and potentially non-uniform test data distributions, our paper aims to develop a principled framework that unifies data distribution, posterior inference, and decision---three key factors in long-tailed classification. Specifically, the differences are:

- Task: [3] assumes the testing distribution to be unknown, while we assume the testing distribution to be known and uniform, which is consistent with most existing long-tail works like [1,2,4].
- Training: [3] is a two-stage model, while our model is one-stage. Our model is easier to implement and more efficient.
- Function of experts: [3] uses different experts to handle different testing distributions (long-tail, balanced, inverse), which means a fixed number of experts. Our model uses "experts" as samples from Bayesian neural networks. Therefore, our model has the flexibility to use more "experts" to pursue better performances, which is impossible in [3].

The above explanation will be added to the final version.

[1] ACE: Ally complementary experts for solving long-tailed recognition in one-shot, CVPR 2021.

[2] Long-tailed recognition by routing diverse distribution-aware experts, ICLR 2021.

[3] Self-Supervised Aggregation of Diverse Experts for Test-Agnostic Long-Tailed Recognition, NeurIPS 2022.

[4] Trustworthy Long-Tailed Classification, CVPR 2022.

[5] The Bayesian Choice, 2007.

\subsection{UTbo[42]}
Thanks for your constructive and helpful comments!

Q1: This paper is not very easy to follow, many technical details are not clear, which makes it difficult to evaluate the contributions. For example, how is the utility function calculated in Section 4.1? Is Eq.2 the final optimization objective? Is there a direct relationship with Eq.1?

A1: Thanks for telling us your concerns! We will address your detailed questions below. In the final version, more explanation to the technical details will be added to improve clarity. We will also release our code to help reproduction.

As shown in Line 152, the values of the utility function $u(j,i)$ can be obtained from the utility matrix $U_{ji}$ at training. The utility matrix $U$ is designed by users depending on different applications, and we show two examples in Figure 1. Our code will help you understand how to compute $U$ technically.

Yes, Eq.2 is the final optimization objective. The code-level computation of Eq.2 is supported by Section 5, where we discuss how to technically compute the train-test discrepancy ratio (Section 5.1), variational distribution $q(\theta)$ (Section 5.2), and the repulsive regularization $KL(q(\theta)||p(\theta))$ (Section 5.3).

Yes, Eq.2 is directly related to Eq.1. Maximizing the "gain" in Eq.2 is equivalent to minimizing the "risk" in Eq.1. This follows similar reasoning presented in Section 3 of [3].

Q2: The relationship between this work and the EM algorithm.

A2: As discussed in Section 4 (Line 130-139), we need to update two things: the variational distribution $q(\theta)$ and the decision $d$, which are dependent on each other. In our framework, inference step (updating $q(\theta)$) and decision step (computing optimal $d$) are conducted alternately, following [3] which adopts a similar variational EM strategy.

Q3: The decision step.

A3: The decision step participates in training but does not modify the parameters. The decision $d^*$ (Section 4.3) is equivalent to the predicted labels of the classifier. During training (Eq.2), we use the true label $y$ because we are updating $q(\theta)$ to make $d^*$ closer to $y$. Therefore, our assumption is, with a good variational distribution, the decisions will be consistent with true labels. We will state this assumption more explicitly in the final version. As for testing, the decision step is directly adopted to compute the predicted labels (last formula in section 4.3).

Q4: What is the proposed network model for the experimental section? The authors should analyze the computational cost.

A4: The implementation details are summarized in appendix D. The model design follows [1,2], with the first few layers shared. All of the particles are updated together using a single objective, so a simple back-propagation works on those shared parameters.

The computational cost of our model is similar to previous ensemble models like [1,2] because the basic architectures are the same. A detailed analysis will be added in the final version.

Q5: Not enough novelty. The authors should focus on analyzing the impact of the utility function on the method under long-tailed distributions, and conduct a theoretical analysis that is closely related to the long-tailed distribution.

A5: We would like to reiterate the novelty of our paper, which we believe is significant and sufficient:

- To the best of our knowledge, this is the first work to formulate long-tailed classification under Bayesian Decision Theory, providing a fresh perspective and unifying key components of long-tailed problems within a single principled framework. It is non-trivial to do so and is in itself a really valuable and novel contribution.
- Under this new framework, we propose a novel loss objective, integrated risk, which incorporates a new repulsive regularization based on the entropy of variational distribution. Moreover, we introduce an efficient particle optimization method that is specially designed to handle large models.
- We extend the evaluation of long-tailed classification to more realistic settings. We seriously consider the misclassificaion of tailed classes due to their sparsity and introduce a new metric FHR (line 348-375).

We have analyzed the impact of utility functions in Table 3\&5, which demonstrate that our tail-sensitive utility improves FHR significantly while maintaining high accuracy. The tail-sensitive utility is important but is just one aspect of our general contributions. Perhaps it is perceived quite narrowly as the focus of our paper. 

[1] Long-tailed recognition by routing diverse distribution-aware experts, ICLR 2021.

[2] Trustworthy Long-Tailed Classification, CVPR 2022.

[3] Approximate inference for the loss-calibrated Bayesian, AISTATS 2011.

